Robust 3D Object Detection in Cold Weather Conditions

Adverse weather conditions can negatively affect LiDAR-based object detectors. In this work, we focus on the phenomenon of vehicle gas exhaust condensation in cold weather conditions. This everyday effect can influence the estimation of object sizes, orientations and introduce ghost object detections, compromising the reliability of the state of the art object detectors. We propose to solve this problem by using data augmentation and a novel training loss term. To effectively train deep neural networks, a large set of labeled data is needed. In case of adverse weather conditions, this process can be extremely laborious and expensive. We address this issue in two steps: First, we present a gas exhaust data generation method based on 3D surface reconstruction and sampling which allows us to generate large sets of gas exhaust clouds from a small pool of labeled data. Second, we introduce a point cloud augmentation process that can be used to add gas exhaust to datasets recorded in good weather conditions. Finally, we formulate a new training loss term that leverages the augmented point cloud to increase object detection robustness by penalizing predictions that include noise. In contrast to other works, our method can be used with both grid-based and point-based detectors. Moreover, since our approach does not require any network architecture changes, inference times remain unchanged. Experimental results on real data show that our proposed method greatly increases robustness to gas exhaust and noisy data.

==> data/tables/mAP/table_ablation_augmentation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
    \caption{Ablation study results on the influence of our gas exhaust data augmentation compared to random noise. The results refer to PointRCNN-Aug evaluated on the DENSE gas-test on the vehicles class.}
    \label{Table:ablation_augmentation}
    \centering
    \begin{adjustbox}{max width=\columnwidth}
        \begin{tabular}{c|c|c|cccc}
            \hline
            \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Random \\ Noise\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Generated \\ Gas Exhaust\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Noise \\ Loss\end{tabular}} & \multicolumn{4}{c}{3D AP}                                                     \\
                                                       &                                            &                                            & Easy                      & Moderate        & Hard           & mAP            \\ \hline
            \xmark                                     & \xmark                                     & \xmark                                     & 56.19                     & 53.68           & 48.87          & 52.92          \\
            \cmark                                     & \xmark                                     & \xmark                                     & 54.76                     & 52.89           & 48.03          & 51.89          \\
            \xmark                                     & \cmark                                     & \xmark                                     & 55.96                     & 53.25           & 48.46          & 52.56          \\
            \cmark                                     & \xmark                                     & \cmark                                     & 56.3                      & 53.88           & 46.86          & 52.35          \\
            \xmark                                     & \cmark                                     & \cmark                                     & \textbf{58.65}           & \textbf{54.38} & \textbf{49.13} & \textbf{54.06} \\ \hline
        \end{tabular}%
    \end{adjustbox}
\end{table}

==> data/tables/mAP/table_ablation_loss.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[t]
    \caption{Ablation study results on the influence of our noise-loss function. The result refer to PointRCNN-Aug evaluated on the DENSE gas-test set on the vehicles class.}
    \label{Table:ablation_loss}
    \centering
    \begin{adjustbox}{max width=\columnwidth}
        \begin{tabular}{c|cccc}
            \hline
            \multirow{2}{*}{$\beta$} & \multicolumn{4}{c}{3D AP}                                                    \\
                                     & Easy                      & Moderate       & Hard           & mAP            \\ \hline
            0                        & 56.19                     & 53.68          & 48.87          & 52.92          \\
            0.01                     & 55.94                     & 53.66          & 48.44          & 52.68          \\
            0.1                      & \textbf{58.65}            & \textbf{54.38} & \textbf{49.13} & \textbf{54.06} \\
            0.5                      & 56.00                     & 53.62          & 48.59          & 52.74          \\
            1                        & 55.45                     & 53.14          & 48.27          & 52.29          \\ \hline
        \end{tabular}%
    \end{adjustbox}
\end{table}

==> data/tables/mAP/table_full_test_set.tex <==
\begin{table*}[t!]
    \caption{Result comparison of the baseline and augmented networks in the test set of the DENSE dataset. For both BEV and 3D the average precision (AP) is measured with 40 recall points and 0.7 IoU threshold on the vehicle class.}
    \label{Table:full_test_set}
    \centering
    \begin{adjustbox}{max width=\textwidth}

        \begin{tabular}{l|cccc|cccc}
            \hline
            \multicolumn{1}{l|}{\multirow{2}{*}{Model}} & \multicolumn{4}{c|}{BEV AP} & \multicolumn{4}{c}{3D AP}                                                                                                        \\
            \multicolumn{1}{c|}{}                            & Easy                        & Moderate                  & Hard           & mAP            & Easy           & Moderate        & Hard           & mAP            \\ \hline
            SECOND   \cite{yan2018second}                    & \textbf{46.65}              & 43.74                     & 40.21          & \textbf{43.53} & \textbf{35.50} & \textbf{32.62}  & \textbf{30.38} & \textbf{32.83} \\
            SECOND-Aug                                       & 46.12                       & \textbf{44.06}            & 40.21          & 43.46          & 35.45          & 32.42           & 30.17          & 32.68          \\
                                                             & -0.53                       & +0.31                     & 0.00           & -0.07          & -0.05          & -0.20           & -0.21          & -0.16          \\ \hline
            PointRCNN    \cite{shi2019pointrcnn}             & \textbf{47.24}              & \textbf{45.24}           & \textbf{40.96} & \textbf{44.48} & 36.47          & 34.98           & \textbf{31.22} & 34.23          \\
            PointRCNN-Aug                                    & 47.12                       & 45.15                     & 40.83          & 44.37          & \textbf{37.95} & \textbf{35.11} & 31.19          & \textbf{34.75} \\
                                                             & -0.12                       & -0.09                     & -0.13          & -0.11          & +1.48          & +0.12           & -0.04          & +0.52          \\ \hline
        \end{tabular}%
    \end{adjustbox}
\end{table*}

==> data/tables/mAP/table_gas_exhaust_test_set.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t!]
    \caption{Result comparison of the baseline and augmented networks in the gas-test set of the DENSE dataset. For both BEV and 3D the average precision (AP) is measured with 40 recall points and 0.7 IoU threshold on the vehicle class.}
    \label{Table:gas_exhaust_test_set}
    \centering
    \begin{adjustbox}{max width=\textwidth}
        \begin{tabular}{l|cccc|cccc}
            \hline
            \multicolumn{1}{l|}{\multirow{2}{*}{Model}} & \multicolumn{4}{c|}{BEV AP} & \multicolumn{4}{c}{3D AP}                                                                                                        \\
            \multicolumn{1}{c|}{}                            & Easy                        & Moderate                  & Hard           & mAP            & Easy           & Moderate        & Hard           & mAP            \\ \hline
            SECOND  \cite{yan2018second}                     & 62.23                       & \textbf{59.60}            & \textbf{54.60} & 58.81          & 56.59          & 51.62           & 46.59          & 51.60          \\
            SECOND-Aug                                       & \textbf{63.61}              & 59.47                     & 54.51          & \textbf{59.20} & \textbf{59.07} & \textbf{54.46}  & \textbf{49.15} & \textbf{54.23} \\
                                                             & +1.38                       & -0.13                     & -0.09          & +0.39          & +2.48          & +2.84           & +2.56          & +2.63          \\ \hline
            PointRCNN    \cite{shi2019pointrcnn}             & 61.99                       & 59.51                     & 52.61          & 58.03          & 56.19          & 53.68           & 48.87          & 52.92          \\
            PointRCNN-Aug                                    & \textbf{64.39}              & \textbf{60.04}            & \textbf{55.17} & \textbf{59.87} & \textbf{58.65} & \textbf{54.38} & \textbf{49.13} & \textbf{54.06} \\
                                                             & +2.40                       & +0.53                     & +2.57          & +1.83          & +2.46          & +0.70           & +0.26          & +1.14          \\ \hline
        \end{tabular}%
    \end{adjustbox}
\end{table*}

==> data/tables/mAP/table_noise_robustness.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t!]
    \caption{Data noise robustness comparison between TANet, PointRCNN and SECOND tested on the full DENSE test set. We express with Aug the networks trained with our proposed method. For both BEV and 3D AP we use 40 recall points and 0.7 IoU threshold.}
    \label{Table:noise_robustness}
    \centering
    \begin{adjustbox}{max width=\textwidth}
        \begin{tabular}{l|c|cccc|cccc}
            \hline
            \multicolumn{1}{l|}{\multirow{2}{*}{Network}} & \multirow{2}{*}{Noise} & \multicolumn{4}{c|}{BEV AP} & \multicolumn{4}{c}{3D AP}                                                                                                                                                                         \\
            \multicolumn{1}{c|}{}                         &                        & \multicolumn{1}{c}{Easy}    & \multicolumn{1}{c}{Moderate} & \multicolumn{1}{c}{Hard} & \multicolumn{1}{c|}{mAP} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Moderate} & \multicolumn{1}{c}{Hard} & \multicolumn{1}{c}{mAP} \\ \hline  \hline
            TANet   \cite{liu2020tanet}                   & \multirow{5}{*}{0}     & 65.16                       & 63.29                        & 57.40                    & 61.95                    & 42.10                    & 40.32                        & 35.76                    & 39.39                   \\ \cline{1-1} \cline{3-10}
            SECOND      \cite{yan2018second}              &                        & \textbf{46.65}              & 43.74                        & 40.21                    & \textbf{43.53}           & \textbf{35.50}           & \textbf{32.62}               & \textbf{30.38}           & \textbf{32.83}          \\
            SECOND-Aug                                    &                        & 46.12                       & \textbf{44.06}               & 40.21                    & 43.46                    & 35.45                    & 32.42                        & 30.17                    & 32.68                   \\ \cline{1-1} \cline{3-10}
            PointRCNN   \cite{shi2019pointrcnn}           &                        & \textbf{47.24}              & \textbf{45.24}               & \textbf{40.96}           & \textbf{44.48}           & 36.47                    & 34.98                        & \textbf{31.22}           & 34.23                   \\
            PointRCNN-Aug                                 &                        & 47.12                       & 45.15                        & 40.83                    & 44.37                    & \textbf{37.95}           & \textbf{35.11}               & 31.19                    & \textbf{34.75}          \\ \hline  \hline
            TANet    \cite{liu2020tanet}                  & \multirow{5}{*}{20}    & 62.22                       & 57.17                        & 54.32                    & 57.90                    & 40.40                    & 36.14                        & 34.28                    & 36.94                   \\ \cline{1-1} \cline{3-10}
            SECOND    \cite{yan2018second}                &                        & 18.50                       & 18.70                        & 17.41                    & 18.20                    & 12.30                    & 11.99                        & 10.76                    & 11.69                   \\
            SECOND-Aug                                    &                        & \textbf{41.84}              & \textbf{38.64}               & \textbf{35.04}           & \textbf{38.51}           & \textbf{30.95}           & \textbf{27.66}               & \textbf{24.60}           & \textbf{27.74}          \\ \cline{1-1} \cline{3-10}
            PointRCNN    \cite{shi2019pointrcnn}          &                        & 42.20                       & 37.94                        & 33.24                    & 37.79                    & 32.15                    & \textbf{29.84}               & \textbf{25.81}           & 29.27                   \\
            PointRCNN-Aug                                 &                        & \textbf{43.11}              & \textbf{39.38}               & \textbf{34.68}           & \textbf{39.06}           & \textbf{32.97}           & 29.78                        & 25.59                    & \textbf{29.45}          \\ \hline  \hline
            TANet   \cite{liu2020tanet}                   & \multirow{5}{*}{50}    & 59.65                       & 55.44                        & 52.26                    & 55.78                    & 38.42                    & 35.04                        & 32.08                    & 35.18                   \\ \cline{1-1} \cline{3-10}
            SECOND  \cite{yan2018second}                  &                        & 9.83                        & 9.77                         & 8.45                     & 9.35                     & 5.91                     & 5.80                         & 5.07                     & 5.59                    \\
            SECOND-Aug                                    &                        & \textbf{40.66}              & \textbf{36.97}               & \textbf{31.82}           & \textbf{36.49}           & \textbf{28.63}           & \textbf{24.76}               & \textbf{21.00}           & \textbf{24.80}          \\ \cline{1-1} \cline{3-10}
            PointRCNN  \cite{shi2019pointrcnn}            &                        & 26.00                       & 21.47                        & 18.83                    & 22.10                    & 21.34                    & 17.53                        & 15.13                    & 18.00                   \\
            PointRCNN-Aug                                 &                        & \textbf{32.49}              & \textbf{28.02}               & \textbf{23.25}           & \textbf{27.92}           & \textbf{24.84}           & \textbf{21.14}               & \textbf{17.93}           & \textbf{21.30}          \\ \hline  \hline
            TANet   \cite{liu2020tanet}                   & \multirow{5}{*}{100}   & 54.86                       & 53.16                        & 46.84                    & 51.62                    & 34.74                    & 33.01                        & 28.50                    & 32.08                   \\ \cline{1-1} \cline{3-10}
            SECOND                                        &                        & 4.73                        & 4.36                         & 3.93                     & 4.34                     & 3.01                     & 2.71                         & 2.30                     & 2.67                    \\
            SECOND-Aug                                    &                        & \textbf{36.49}              & \textbf{31.65}               & \textbf{26.65}           & \textbf{31.59}           & \textbf{25.34}           & \textbf{21.29}               & \textbf{17.87}           & \textbf{21.50}          \\ \cline{1-1} \cline{3-10}
            PointRCNN     \cite{shi2019pointrcnn}         &                        & 9.37                        & 7.08                         & 4.83                     & 7.09                     & 6.47                     & 4.67                         & 4.42                     & 5.18                    \\
            PointRCNN-Aug                                 &                        & \textbf{14.10}              & \textbf{11.14}               & \textbf{9.04}            & \textbf{11.43}           & \textbf{10.85}           & \textbf{8.25}                & \textbf{6.41}            & \textbf{8.51}           \\ \hline
        \end{tabular}%
    \end{adjustbox}
\end{table*}

==> data/tables/tmp.tex <==
\begin{table}[t!]
    \caption{TP1}
    \label{Table:full_test_set}
    \centering
    \begin{adjustbox}{max width=\columnwidth}

        \begin{tabular}{l|ccc|ccc}
            \hline
            \multicolumn{1}{l|}{\multirow{2}{*}{Model}} & \multicolumn{3}{c|}{BEV AP} & \multicolumn{3}{c}{3D AP}                                                                     \\
            \multicolumn{1}{c|}{}                       & Easy                        & Moderate                  & Hard           & Easy           & Moderate       & Hard           \\ \hline
            SECOND                 & \textbf{46.65}              & 43.74                     & 40.21          & \textbf{35.50} & \textbf{32.62} & \textbf{30.38} \\
            SECOND-Aug                                  & 46.12                       & \textbf{44.06}            & 40.21          & 35.45          & 32.42          & 30.17          \\  
            \rowcolor{LightCyan}                                            & -0.53                       & +0.31                     & 0.00           & -0.05          & -0.20          & -0.21         \\  \hline
            PointRCNN          & \textbf{47.24}              & \textbf{45.24}            & \textbf{40.96} & 36.47          & 34.98          & \textbf{31.22} \\
            PointRCNN-Aug                               & 47.12                       & 45.15                     & 40.83          & \textbf{37.95} & \textbf{35.11} & 31.19          \\
            \rowcolor{LightCyan}                                            & -0.12                       & -0.09                     & -0.13          & +1.48          & +0.12          & -0.04          \\   \hline
        \end{tabular}%
    \end{adjustbox}
\end{table}


==> data/tables/tmp2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t!]
    \caption{Data noise robustness comparison between TANet~\cite{liu2020tanet}, PointRCNN~ and SECOND~ tested on the full DENSE~\cite{bijelic2020seeing} test set. We express with Aug the networks trained with our proposed method.  Both BEV AP and 3D AP are measured with $40$ recall points and $0.7$ IoU threshold on the vehicle class.}
    \label{Table:noise_robustness}
    \centering
    \begin{adjustbox}{max width=\textwidth}
        \begin{tabular}{l|c|ccc|ccc}
            \hline
            \multicolumn{1}{l|}{\multirow{2}{*}{Model}} & \multirow{2}{*}{Noise} & \multicolumn{3}{c|}{BEV AP}       & \multicolumn{3}{c}{3D AP}                                                                                                                     \\
            \multicolumn{1}{c|}{}                       &                        & \multicolumn{1}{c}{Easy}          & \multicolumn{1}{c}{Moderate} & \multicolumn{1}{c|}{Hard} & \multicolumn{1}{c}{Easy} & \multicolumn{1}{c}{Moderate} & \multicolumn{1}{c}{Hard} \\ \hline
            TANet                                       & \multirow{5}{*}{0}     & 65.16                             & 63.29                        & 57.40                     & 42.10                    & 40.32                        & 35.76                    \\ \cline{1-1} \cline{3-8}
            SECOND                                      &                        & \textbf{46.65}                    & 43.74                        & 40.21                     & \textbf{35.50}           & \textbf{32.62}               & \textbf{30.38}           \\
            SECOND-Aug                                  &                        & 46.12         & \textbf{44.06}               & 40.21                     & 35.45                    & 32.42                        & 30.17                    \\
            % PointRCNN                                   &                        & \textbf{47.24}              & \textbf{45.24}               & \textbf{40.96}            & 36.47                    & 34.98                        & \textbf{31.22}           \\
                                                        &                        & \rowcolor{LightCyan} -0.53                             & +0.32                         & 0.00                      & -0.05                    & -0.20                        & -0.21                    \\ \hline  \hline
            TANet                                       & \multirow{5}{*}{20}    & 62.22                             & 57.17                        & 54.32                     & 40.40                    & 36.14                        & 34.28                    \\ \cline{1-1} \cline{3-8}
            SECOND                                      &                        & 18.50                             & 18.70                        & 17.41                     & 12.30                    & 11.99                        & 10.76                    \\
            SECOND-Aug                                  &                        & \textbf{41.84}                    & \textbf{38.64}               & \textbf{35.04}            & \textbf{30.95}           & \textbf{27.66}               & \textbf{24.60}           \\
            % PointRCNN                                   &                        & 42.20                       & 37.94                        & 33.24                     & 32.15                    & \textbf{29.84}               & \textbf{25.81}           \\
                                                        &                        & \rowcolor{LightCyan}   +23.34 & +19.94                        & +17.63                     & +18.65                    & +15.67                        & +13.84                    \\ \hline  \hline
            TANet                                       & \multirow{5}{*}{50}    & 59.65                             & 55.44                        & 52.26                     & 38.42                    & 35.04                        & 32.08                    \\ \cline{1-1} \cline{3-8}
            SECOND                                      &                        & 9.83                              & 9.77                         & 8.45                      & 5.91                     & 5.80                         & 5.07                     \\
            SECOND-Aug                                  &                        & \textbf{40.66}                    & \textbf{36.97}               & \textbf{31.82}            & \textbf{28.63}           & \textbf{24.76}               & \textbf{21.00}           \\
                                                        &                        & \rowcolor{LightCyan} +30.83        & +27.20                        & +23.37                     & +22.72                    & +18.96                        & +15.93                    \\ \hline  \hline
            TANet                                       & \multirow{5}{*}{100}   & 54.86                             & 53.16                        & 46.84                     & 34.74                    & 33.01                        & 28.50                    \\ \cline{1-1} \cline{3-8}
            SECOND                                      &                        & 4.73                              & 4.36                         & 3.93                      & 3.01                     & 2.71                         & 2.30                     \\
            SECOND-Aug                                  &                        & \textbf{36.49}                    & \textbf{31.65}               & \textbf{26.65}            & \textbf{25.34}           & \textbf{21.29}               & \textbf{17.87}           \\
            % PointRCNN                                   &                        & 9.37                        & 7.08                         & 4.83                      & 6.47                     & 4.67                         & 4.42                     \\
                                                        &                        & \rowcolor{LightCyan} +31.76        & +27.29                        & +22.72                     & +22.33                    & +18.58                        & +15.57                    \\ \hline
        \end{tabular}%
    \end{adjustbox}
\end{table*}
